RVI-SAC: Average Reward Off-Policy Deep Reinforcement Learning

In this paper, we propose an off-policy deep reinforcement learning (DRL) method utilizing the average reward criterion. While most existing DRL methods employ the discounted reward criterion, this can potentially lead to a discrepancy between the training objective and performance metrics in continuing tasks, making the average reward criterion a recommended alternative. We introduce RVI-SAC, an extension of the state-of-the-art off-policy DRL method, Soft Actor-Critic (SAC), to the average reward criterion. Our proposal consists of (1) Critic updates based on RVI Q-learning, (2) Actor updates introduced by the average reward soft policy improvement theorem, and (3) automatic adjustment of Reset Cost enabling the average reward reinforcement learning to be applied to tasks with termination. We apply our method to the Gymnasium's Mujoco tasks, a subset of locomotion tasks, and demonstrate that RVI-SAC shows competitive performance compared to existing methods.

==> plotter/output/main_result.tex <==
\begin{table}
\caption{Max Average Return over 10 trials of 1 million time steps.}
\label{tab:main_result}
\begin{tabular}{lllllll}
\toprule
 & ARO-DDPG & ATRPO & RVI-SAC & SAC-0.97 & SAC-0.99 & SAC-0.999 \\
\midrule
Ant & 2073.89±186.00 & 959.25±18.57 & 6104.14±199.33 & 4855.87±1257.02 & 4511.20±605.98 & 1948.53±875.50 \\
\bottomrule
\end{tabular}
\end{table}


==> sections/ja/01_introduction.tex <==
\section{Introduction}

モデルフリー強化学習は最適な方策を環境との相互作用を通して獲得することを目的とする枠組みである．
特に方策や価値関数をNeural Networkで近似するDeep Reinforcement Learning (DRL)は近年急速に発展しており，Mujoco\cite{todorov2012mujoco}タスクのような高次元の連続行動空間を持つタスクを解くことを可能にした．
高次元の連続行動空間を持つタスクに適用するDRL手法として，TRPO\cite{Schulman2015TRPO}，PPO\cite{Schulman2017PPO}，DDPG\cite{Silver2014DPG,Lillicrap2016DDPG}，TD3\cite{Fujimoto2018TD3}，SAC\cite{Haarnoja2018SAC,Haarnoja2018SACv2}などが良く知られており，これらの手法は割引報酬基準が用いられている．
割引報酬基準は様々な種類のMDPで定式化されるタスクに適用可能である\cite{Puterman1994MDP}．
特にロボットロコモーションやAccess Control Queing Taskのようなエピソードに明確な区切りのないcontinuing taskにおいて，割引率はinfinite horizon returnを有界に抑える役割を持つ．
しかし，割引は現在時刻に近い報酬を遠い報酬と比べて優先させるという，continuing taskにおいては望ましくない効果を持つ．
この効果を緩和するための一つの方法として、割引係数を1に近づけることがありますが、一般的に大きな割引係数は不安定さを引き起こすことが知られています．\cite{Fujimoto2018TD3}

近年は，割引報酬基準を用いない手法として平均報酬基準が注目されはじめている．
平均報酬型強化学習は，continuing taskにおいてinfinite horizon rewardの時間平均の最大化を目的とする手法であり，continuing taskにおいては，割引報酬基準よりも平均報酬基準のほうが，より自然である．
DRLの文脈においても，数少ないながら平均報酬基準を用いた手法が提案されている．
特に，割引報酬基準を用いたstate-of-the-artなOn-policy DRL手法であるTRPO/PPOを平均報酬基準に拡張したATRPO\cite{Yiming2021ATRPO}/APO\cite{DBLP:journals/corr/abs-2106-08322}は，
Mujoco\cite{todorov2012mujoco}タスクにおいて，割引報酬基準を用いた手法と同等以上の性能を示すことが報告されている．

平均報酬基準と，On-policyよりサンプル効率が良いことが一般的にしれらているOff-policy手法を組み合わせた研究の数は少ない．
平均報酬基準を用いたOff-policy手法として，R-learning, RVI Q-learning\cite{Abounadi2001RVI}，Differential Q-learnig\cite{AverageRewardQLearning}，CSV Q-learningなど理論的研究やテーブル型の手法は複数存在する.
しかし，我々の知る限り，平均報酬基準を用いたOff-policy DRL手法は，決定的な方策を最適化するARO-DDPG\cite{ARO-DDPG}のみである．
割引率を用いたDRLの研究では，方策のエントロピーが加えられた目的に対して確率的方策を最適化することで探索を効率化し，サンプル効率を大幅に改善できること知られており\cite{Haarnoja2018SAC}，
entropy-augumented rewardのコンセプトを用いたOff-policy手法は成功を収めている．
しかし，平均報酬基準において，このコンセプトを適用したOff-policy DRL手法は提案されていない．

我々の目的は，平均報酬基準でentropy-augumented rewardのコンセプトを適用したOff-policy Actor-Critic DRL手法であるRVI-SACを提案することである．
我々の提案手法の中では，Criticの更新には，RVI Q-learningをベースとした，新たなQ-Networkの更新手法を用いる．
RVI Q-learningは，ARO-DDPGでベースとされていたDifferential Q-learningと違い，Q関数の収束するポイントを一意に定めることができる．\cite{Abounadi2001RVI,Wan2020DifferentialQLearning}
我々は，RVI Q-learningをNeural Networkを用いた手法にナイーブに拡張した際に生じる問題点を指摘し，その問題点を解決するためにDelayed f(Q) Updateという工夫を施すことにより，RVI Q-learningをNeural Networkに拡張可能にしている．
また，Delayed f(Q) Updateを用いたRVI Q-learningのテーブル型の問題設定におけるODEを用いたasymptotic convergence analysisも提供している．
Actorの更新に関して，SACのsoft policy improvement theoremをベースとした，average reward soft policy improvement theoremを導出することにより，soft average rewardの改善を保証する方策の更新手法を新たに構築する．

我々の提案する方法は，ロボットロコモーションタスク，例えばMujocoのWalker2d，Humanoid，Hopper，Antのような，ロボットが転倒してエピソードを終了する可能性があるような，純粋なcontinuing taskではないタスクに対して平均報酬型強化学習を適用する際の課題に対処する．
平均報酬型強化学習はinfinite horizon rewardの時間平均を最適化するため，これらのタスクで発生する可能性があるエピソードの終了は許容されない．
我々は，このようなタスクにおいても，ATRPOと同様に，転倒後にpenalty reward(reset cost)を与え，環境をリセットする処理を導入する．
ATRPOではReset Costはハイパーパラメータとして与えられていた．
しかし，適切なReset Costの大きさは，タスクの報酬スケールに依存し，Reset Costの設定が最終的な性能に影響する可能性がある．
我々の提案手法では，平均報酬を最大化を目的関数とし，リセットが発生する頻度という報酬スケールに依存しない量を制約条件とする制約付き最適化問題を解くことで，Reset Costを自動調整する．

我々の主な貢献は以下の通りである．
\begin{itemize}
  \item 我々は，平均報酬基準において，entropy-augumented average rewardに対して，確率的方策を最適化する新たなOff-policy Actor-Critic DRL手法，RVI-SACを提案する．
        この手法は，RVI Q-learningをベースとした，新たなQ-Networkの更新手法と，average reward soft policy improvement theoremによって導かれる，方策更新手法によって構成される．
  \item 我々は，提案手法を，continuingとepisodicの両方の性質を持つタスクに適用するために，環境のResetを導入し，その際のペナルティ(reset cost)を自動調整する手法を提案する． % 制約付き最適化の話をここにも書く．
  \item 我々の提案手法が，様々な割引率を設定したSACや，既存の平均報酬型のDRL手法と比べて，Competitiveな性能を示すことをMujocoを用いたベンチマーク実験によって示す．
\end{itemize}

==> sections/ja/02_preliminaries.tex <==
\section{Preliminaries}

\subsection{Notation}

本論文では，以下に示す数学的記法を用いる．
\begin{itemize}
  \item $e$は全ての要素が1のベクトルを表す．
  \item $D_{\text{KL}}(p|q)$は，Kullback-Leibler divergenceを表し，確率分布$p,q$間で$D_{\text{KL}}(p | q) = \sum_x p(x) \log\frac{p(x)}{q(x)}$と定義される．
  \item ここで，$\mathbbm{1}(\text{"some condition"})$は指示関数であり，"some condition"を満たす場合は$1$，それ以外は$0$の値をとる．
  \item $\|\cdot\|_\infty$はsup-normを表す．
\end{itemize}


\subsection{Markov Decision Process}

我々は，環境とエージェントの相互作用をMarkov Decision Process (MDP) $\mathcal{M} = (\mathcal{S}, \mathcal{A}, r, p)$で定義する．
ここで，$s \in \mathcal{S}$は状態集合，$a \in \mathcal{A}$は行動集合，$r: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}, |r(\cdot, \cdot)| \leq \|r\|_\infty $は報酬関数，
$p: \mathcal{S} \times \mathcal{A} \times \mathcal{S} \to [0, 1]$は状態遷移関数を表す．
一連の離散的な時間ステップ$t=0,1,2,\ldots$において，エージェントはMDPの状態$S_t \in \mathcal{S}$を受け取り，行動$A_t \in \mathcal{A}$を選択する．
その後，環境から報酬$R_t = r(S_t, A_t)$および次の状態$S_{t+1} \in \mathcal{S}$を受け取り，これを繰り返す．
状態遷移関数は，$p\left(s^{\prime}\mid s, a\right) := \operatorname{Pr}\left(S_{t+1}=s^{\prime} \mid S_t=\right.$ $\left.s, A_t=a\right)$として，すべての$s, s^{\prime} \in \mathcal{S}, a \in \mathcal{A}$に対して定義される．
また，我々は行動選択の基準として，定常なマルコフ方策$\pi: \mathcal{S} \times \mathcal{A} \rightarrow [0, 1]$を用いる．
これは，状態$s \in \mathcal{S}$において行動$a \in \mathcal{A}$を選択する確率を表し，$\pi(a|s) := \operatorname{Pr}\left(A_t=a \mid S_t=s\right)$と定義される．

\subsection{Average Reward Reinforcement Learning}
\label{sec:average_reward_reinforcement_learning}

我々は，以降の議論を簡単にするため，平均報酬型強化学習を適用するMDPに以下を仮定する．
\begin{assumption}
  \label{assumption:ergodic}
  任意の方策$\pi$に対して，MDP $\mathcal{M}$はergodicである．
\end{assumption}
この仮定の下では，方策$\pi$に対して，定常状態分布$d_{\pi}(s)$が存在する．行動も含めた分布を$d_\pi(s, a) = d_\pi(s) \pi(s|a)$と表記する．

ある方策$\pi$に対する平均報酬は以下のように定義される．
\begin{equation}
  \label{eq:average_reward}
  \rho^{\pi} := \lim_{T \rightarrow \infty} \frac{1}{T} \underE{\pi}{\sum_{t=0}^{\infty} R_t} = \sum_{s \in \mathcal{S}} d_\pi(s,a) r(s,a)
\end{equation}
平均報酬型強化学習における最適方策は，平均報酬の定義より，
\begin{equation}
  \pi^* = \argmax_{\pi} \rho^{\pi}
\end{equation}
となる．

平均報酬型の行動価値関数は以下のように定義される．
\begin{equation}\label{eq:average_reward_Q}
  Q^\pi(s,a) := \underE{\pi}{\sum_{t=0}^{\infty} (R_t - \rho^\pi) | S_0 = s, A_0 = a}
\end{equation}

平均報酬型の最適ベルマン方程式は以下のようになる．
\begin{equation}
  \label{eq:average_reward_optimal_bellman_equation}
  \begin{aligned}
    Q(s, a) = r(s, a) - \rho + \sum_{s' \in \mathcal{S}} p(s'|s, a) \max_{a'} Q(s', a'), \\
    \forall (s,a) \in \mathcal{S} \times \mathcal{A}
  \end{aligned}
\end{equation}
既存研究(e.g. \citet{Puterman1994MDP})より，この方程式には以下のような性質があることがわかっている．
\begin{itemize}
  \item $\rho$に関して，$\rho = \rho^{\pi^*}$と解が一意に定まる．
  \item $Q(s,a)$に関して，任意の定数$c \in \mathbb{R}$上で，$q(s,a) = Q^{\pi^*}(s,a) + c$と解が定まる．
  \item 上記の方程式の解$Q$に対して，決定的方策$\mu(s) = \argmax_{a} q(s,a)$は最適方策の一つである．
\end{itemize}
以下，$\rho^{\pi^*} = \rho^*$と表記する．


\subsection{RVI Q-learning}
\label{sec:RVI_Q_learning}

RVI Q-learning\cite{Konda1999ActorCriticSA,Wan2020DifferentialQLearning}は，平均報酬型強化学習におけるQ-learningの一つであり，テーブル型で表されるQ関数に対して，以下のようなiterationを行う.
\begin{eqnarray}
  \label{eq:RVI_Q_learning}
  \begin{aligned}
     & Q_{t+1}(S_t, A_t)  = Q_t(S_t, A_t) +                                          \\
     & \alpha_t \left( R_t - f(Q_t) + \max_{a'} Q_t (S_{t+1}, a') - Q_t(S_t, A_t)\right)
  \end{aligned}
\end{eqnarray}
一般化されたRVI Q-learningの収束の証明\cite{Wan2020DifferentialQLearning}より，関数$f$は以下のような仮定を満たす任意の関数である．
\begin{assumption}[From \citet{Abounadi2001RVI}]
  $f: \mathbb{R}^{|\mathcal{S} \times \mathcal{A}|} \rightarrow \mathbb{R}$ is Lipschitz and there exists some $u>0$ such that $\forall c \in \mathbb{R}$ and $x \in \mathbb{R}^{|\mathcal{S} \times \mathcal{A}|}, f(e)=u$, $f(x+c e)=f(x)+c u$ and $f(c x)=c f(x)$,
\end{assumption}
実際には$f$として，任意の状態/行動ペア$(S,A)$をReference Stateとした$f(Q) = Q(S,A), \max_{a} Q(S,a)$や，
全状態/行動ペアに関する和$f(Q) = \sum_{(s,a) \in \mathcal{S}\times\mathcal{A}} Q(s,a), \sum_{s \in \mathcal{S}} \max_{a} Q(s,a)$などがよく用いられる．

このアルゴリズムは，ある適切な仮定のもと，$Q_t$が確率1で一意に定まる$q^*$に収束し，$q^*$は式\ref{eq:average_reward_optimal_bellman_equation}の最適ベルマン方程式に加えて，
$$
  \rho^* = f(q^*)
$$
を満たすことが示されている\cite{Wan2020DifferentialQLearning}．

==> sections/ja/03_proposal.tex <==
\section{Proposed Method}

我々は今，平均報酬を基準とした新たなActor-Critic型の深層強化学習手法を提案する．
そのために，\ref{sec:RVI_Q_learning_based_Q_Network_update}節では，RVI Q-learningをベースとしたCriticの更新手法を示し，
\ref{sec:Average_Reward_Soft_Policy_Improvement_Theorem}節では，平均報酬を尺度としたActorの更新手法をSoft Actor-Critic\cite{Haarnoja2018SAC}に基づいて示す．
また，\ref{sec:Automatic_Reset_Cost_Adjustment}節では，転倒状態を持つロコモーションタスクのような，純粋なcontinuingタスクではない問題に対しても平均報酬型強化学習を適用するための手法を示す．

\subsection{RVI Q-learning based Q-Network update}
\label{sec:RVI_Q_learning_based_Q_Network_update}


式\ref{eq:RVI_Q_learning}に基づいたアルゴリズムを，Neural Networkによって表現されたQ関数の更新に直接拡張する．
Neural NetworkベースのQ-learning手法の伝統的な方法に従うと，
パラメーター$\phi$を持つQ-Network $Q_{\phi}$に対して，
ターゲット
$$
  Y(r, s') = r - f(Q_{\phi'}) + \max_{a'} Q_{\phi'}(s', a'),
$$
を用い，
次の損失関数を最小化するように$\phi$を更新する．
$$
  \text{loss}(\phi) = \frac{1}{|\mathcal{B}|} \sum_{(s, a, r, s') \in \mathcal{B}}\left(Y(r, s') - Q_{\phi}(s, a)\right)^2
$$
ここで$\mathcal{B}$は，学習中に得られた経験$(S_t, A_t, R_t,S_{t+1})$を蓄積するReplay Buffer $\mathcal{D}$から一様にサンプルされたミニバッチ$\mathcal{B}$で，$\phi'$はターゲットネットワーク\cite{Mnih2013DQN}のパラメータである．
この更新を行う上で，以下の2つの点を考慮する必要がある．

1つ目の考慮点は，関数$f$の選択である．
\ref{sec:RVI_Q_learning}節では，テーブル型のQ-learningにおいて，Reference State $(S, A) \in \mathcal{S} \times \mathcal{A}$を用いた方法や，全状態/行動ペアに対する和を計算する方法が一般的であることを述べた．
Reference Stateを用いる方法は，連続な状態/行動空間を持つ問題にも容易に拡張可能である．しかし，Reference Stateへの訪問頻度やそのQ値の精度にアルゴリズム全体の性能が依存する懸念がある．\cite{Wan2020DifferentialQLearning}
一方で，全状態/行動ペアに対する和を計算する方法は，Reference Stateが不要であるものの，Neural Networkを用いた場合には$f(Q_{\phi'})$の値が直接計算が出来ない．
これらの問題を回避するため，我々はミニバッチ$\mathcal{B}$を用い，以下の式\ref{eq:F_Sampled}で示される値$f(Q_{\phi'}; \mathcal{B})$を$f(Q_{\phi'})$の代替として採用する．
\begin{equation}
  \label{eq:F_Sampled}
  f(Q_{\phi'}; \mathcal{B}) = \frac{1}{|\mathcal{B}|} \sum_{(s, a, r, s') \in \mathcal{B}} \max_{a'} Q_{\phi'}(s', a')
\end{equation}
式\ref{eq:F_Sampled}は，$f(Q_{\phi'})$を，
\begin{equation}\label{eq:F_Sampled_unbiased_estimator}
  f(Q_{\phi'}) = \underE{s \sim d_{b}(\cdot)}{\max_{a} Q_{\phi'}(s, a)}
\end{equation}
と設定したときの不偏推定値となる．ここで，$b$はOff-policy手法におけるbehavior policyを表し，$d_{b}(\cdot)$はbehavior policy $b$における定常状態分布を表す．
我々の手法では，式\ref{eq:F_Sampled},\ref{eq:F_Sampled_unbiased_estimator}のような設定を用いたが，ある確率変数$X$に対して
\begin{equation}
  \label{eq:F_Sampled_general}
  f(Q_{\phi'}) = \underE{X}{f(Q_{\phi'}; X)}
\end{equation}
を満たす任意の設定に，この議論は適用可能である．
以上より，Q-Networkの更新に用いられるターゲット値は，
\begin{equation}
  \label{eq:Q_Network_target1}
  Y(r, s'; \mathcal{B}) = r - f(Q_{\phi'}; \mathcal{B}) + \max_{a'} Q_{\phi'}(s', a')
\end{equation}
となる．

2つ目の考慮点は，サンプル値$f(Q_{\phi'}; \mathcal{B})$(式\ref{eq:F_Sampled})の分散によって引き起こされるターゲット値(式\ref{eq:Q_Network_target1})の分散が，学習を不安定にすることである．
特に，Q関数の分散が大きい場合，この問題が顕著になるり，
Q値の大きな分散は，ターゲット値の分散を増加させ，結果としてQ値の分散を更に大きくするという悪循環を引き起こす可能性がある．
ターゲット値の分散を抑制するため，我々は\textbf{Delayed f(Q) Update}を提案する．
Delayed f(Q) Updateは，$f(Q_{\phi'}; \mathcal{B})$の代わりに，以下のような式で更新される値$\xi_t$を用いる．
$$
  \xi_{t+1} = \xi_{t} + \beta_t \left(f(Q_{\phi'};\mathcal{B}) - \xi_t\right)
$$
ここで，$\beta_t$は$\xi_t$の学習率を表す．
また，$\xi_t$を用いた新たなターゲット値は以下のようになる．
$$
  Y(r, s'; \xi_t) = r - \xi_t + \max_{a'} Q_{\phi'}(s', a')
$$
ここで$\xi_t$は$f(Q_{\phi'}; \mathcal{B})$の平滑化された値となり，この更新法によりターゲット値の分散が低減されることが期待される．

\textbf{Theoretical Analysis of Delayed f(Q) Update}

Delayed f(Q) Updateを用いたQ-Networkの更新手法を，テーブル型のQ-learningに基づくアルゴリズムに引き戻すと，以下のように書き表される．
\small
\begin{equation}
  \begin{aligned}
    \label{eq:RVI_Q_learning_with_Delayed_fQ_Update}
    Q_{t+1}(S_t, A_t) & = Q_{t}(S_t, A_t) +                                                                  \\
                      & \alpha_{t} \left(R_t - \xi_t + \max_{a'} Q_{t}(S_{t+1}, a') - Q_{t}(S_t, A_t)\right) \\
    \xi_{t+1}         & = \xi_{t} + \beta_t \left(f(Q_t; X) - \xi_t\right)
  \end{aligned}
\end{equation}
\normalsize
この更新式は，two time scaleでasynchrousなstochastic approximation(SA)の特殊化である．\cite{xxx}
$\frac{\alpha_t}{\beta_t} \rightarrow 0$となるような適切な学習率を選択することで，
式\ref{eq:RVI_Q_learning_with_Delayed_fQ_Update}の$\xi_t$の更新が$Q_t$の更新に比べて速いと見ることができる．
そのため，$\xi_t$は"相対的に定数"となるため，$f(Q_t)$と同じと見ることができ，式\ref{eq:RVI_Q_learning}と同じと見ることができる．
このアルゴリズムの収束に関しては，Appendix \ref{sec:convergence_proof_of_RVI_Q_learning_with_Delayed_fQ_Update}で議論する．

\subsection{Average Reward Soft Policy Improvement Theorem}
\label{sec:Average_Reward_Soft_Policy_Improvement_Theorem}
我々は、方策の更新手法として、soft actor-criticにおける方策の更新をベースとして採用する \cite{Haarnoja2018SAC}．
この方法は、割引率$\gamma \in (0,1)$と既存の方策$\pi$に対して，
\begin{equation}\label{eq:soft_Q_function}
  \begin{aligned}
     & Q^{\pi, \gamma}(s, a)  :=                                                                                   \\
     & \underE{\pi}{\sum_{t=1}^{\infty} \gamma^t \left(R_t - \log \pi(A_{t+1}|S_{t+1})\right) | S_0 = s, A_0 = a},
  \end{aligned}
\end{equation}
で定義されるsoft-Q関数を用いて以下のように方策を更新する．
\begin{equation}\label{eq:soft_policy_update}
  \begin{aligned}
    \pi_{\text{new}}(\cdot|s) = \argmin_{\pi \in \Pi} D_{\text{KL}} \left( \pi(\cdot|s) \middle| \frac{\exp{(Q^{\pi_{\text{old}}, \gamma}(s, \cdot))}}{Z^{\pi_{\text{old}}}(s)} \right), \\
    \forall s \in \mathcal{S}.
  \end{aligned}
\end{equation}
パーティション関数$Z^{\pi_{\text {old}}}\left(\mathbf{s}_t\right)$は分布を正規化するために用いられており，新しい方策に関する勾配には寄与しないため無視できる(see \citet{Haarnoja2018SAC})．
$\Pi$は方策の集合，例えば Gaussian policyのようなparametrized family，を表す．
soft policy improvement theoremによると\cite{Haarnoja2018SAC}，式\eqref{eq:soft_policy_update}に基づく更新後の方策$\pi_{\text{new}}$について、$Q^{\pi_{\text{new}}, \gamma}(s, a) \geq Q^{\pi_{\text{old}}, \gamma}(s, a), \forall (s, a) \in \mathcal{S} \times \mathcal{A}$が成り立つ，つまり方策が改善することが示されている．
soft actor-criticのActorの更新ルールはこの定理に基づき構築される．
また，entropy augumented reward $R_t^{\text{ent}} := R_t - \underE{s' \sim p(\cdot|S_t, A_t)\\ a \sim \pi(\cdot|S_t)}{\log \pi(a|s')}$を定義すると，式\ref{eq:soft_Q_function}のQ関数は，
$Q^{\pi, \gamma}(s, a):=\underE{\pi}{\sum_{t=1}^{\infty} \gamma^t R_t^{\text{ent}} | S_0 = s, A_0 = a}$と書き直すことができるため，
Criticの更新はstandardなdiscounted Q-learningの枠組みを適用できることが示されている．\cite{Haarnoja2018SAC}


平均報酬型強化学習の文脈では，soft average rewardは次のように定義される．
\begin{equation}
  \label{eq:soft_average_reward}
  \rho^{\pi}_{\text{soft}} = \lim_{T \rightarrow \infty} \frac{1}{T} \underE{\pi}{\sum_{t=0}^{\infty} R_t - \log \pi(A_{t}|S_{t})}
\end{equation}
これに対して，average reward type soft-Q関数を次のように定義する．
\small
\begin{equation}
  \label{eq:soft_average_reward_Q}
  \begin{aligned}
     & Q^{\pi}(s, a) :=                                                                                                 \\
     & \underE{\pi}{\sum_{t=0}^{\infty} R_t - \rho^{\pi}_{\text{soft}} - \log \pi(A_{t+1}|S_{t+1}) | S_0 = s, A_0 = a }
  \end{aligned}
\end{equation}
\normalsize
式\ref{eq:soft_average_reward_Q}より，ソフト行動価値関数は報酬から平均報酬を引いた値の累積和の期待値のであるため，
割引率を用いたsoft actor-criticにおけるpolicy improvement theoremでの議論にある，
$Q^{\pi_{\text{new}}}(s, a) \geq Q^{\pi_{\text{old}}}(s, a)$という関係は方策の改善を保証しない．
我々はソフト平均報酬$\rho^\pi_{\text{soft}}$を尺度とした新たなaverage reward soft policy improvement示す．
\begin{theorem}[average reward soft policy improvement]
  Let $\pi_{\text {old }} \in \Pi$ and let $\pi_{\text {new }}$ be the optimizer of the minimization problem defined in Equation \ref{eq:soft_policy_update}.
  Then $\rho^{\pi_{\text {new }}} \geq \rho^{\pi_{\text {old }}}$ with $|\mathcal{A}|<\infty$.
\end{theorem}
\begin{proof}
  See Apendix.
\end{proof}
この結果は，ソフト平均報酬を尺度とした提案手法でも，soft actor-criticと同じ，Actorの更新ルールによって，方策が改善することを示している．
また，entropy augumented reward $R_t^{\text{ent}}$とentropy augumented Q関数$Q^{\pi, \text{ent}}(s, a)$を，
\begin{eqnarray}
  R_t^{\text{ent}} := R_t - \log \pi(A_t|S_t)\\
  Q^{\pi, \text{ent}}(s, a) := Q^{\pi}(s, a) - \log \pi(A_t|S_t) \label{eq:soft_average_reward_Q_ent}
\end{eqnarray}
と定義すると，
式\ref{eq:soft_average_reward_Q}のQ関数は，$Q^{\pi, \text{ent}}(s, a) := \underE{\pi}{\sum_{t=0}^{\infty} R_t^{\text{ent}} - \rho^{\pi}_{\text{soft}} | S_0 = s, A_0 = a }$
と書き直すことができる．
この式は平均報酬型のQ関数の定義式\ref{eq:average_reward_Q}と同じ形をしており，Criticの更新は平均報酬型強化学習におけるQ-learningの枠組みを適用できる．
% \begin{theorem}[average reward soft policy improvement]
%   Let $\pi_{\text {old }} \in \Pi$ and let $\pi_{\text {new }}$ be the optimizer of the minimization problem defined in Equation \ref{eq:soft_policy_update}.
%   Then $\rho^{\pi_{\text {new }}} \geq \rho^{\pi_{\text {old }}}$ with $|\mathcal{A}|<\infty$.
% \end{theorem}
% \begin{proof}
%   See Apendix.
% \end{proof}

\subsection{Automatic Reset Cost Adjustment}
\label{sec:Automatic_Reset_Cost_Adjustment}

本Sectionでは，転倒によってエピソードが終了する可能性があるようなロコモーションタスクのような，純粋なcontinuingタスクではないタスクを平均報酬基準で扱う際の課題に対処する．
平均報酬型強化学習は，エピソードが終了しないcontinuousタスクを仮定している．
これは，平均報酬は無限区間で定義されており，エピソードの終了後はエージェントは報酬0を受け取り続けるため，平均報酬が0となり，方策を適切に評価できないためである．
しかし，多くのタスク，例えばロコモーションタスクでは，方策の学習が十分ではない学習初期において，エージェントが転倒しエピソードが終了するが，学習が進むにつれエピソードが終了しなくなるようなepisodicタスクとcontinuingタスク両方の性質を併せ持つようなタスクが存在する．

我々は，このようなタスクにも平均報酬型強化学習を適用するため，ATRPO\cite{Yiming2021ATRPO}において用いられている，環境のResetとReset Costを導入する．
環境のResetとは，エージェントの転倒などでエピソードが終了しても，環境を初期化することによって，エピソードが継続しているものとして扱うことである．
また，Reset Costとは環境をResetしたこと対して与えられるペナルティ報酬$-r_{\text{cost}}$（ただし$r_{\text{cost}} > 0$）である．
つまり，ある状態$s$においてエピソードが終了した後も，何かしら行動$a$を選択し，環境を初期化して初期状態$s_0$を観測することにより，経験$(s, a, -r_{\text{cost}}, s_0)$を得て，エピソードを継続したものとして扱う．

ATRPOにおいては，Mujoco環境に対する実験で$r_{\text{cost}}=100$と固定していた．
しかし，環境や報酬のスケールによって適切なReset Costは変化し，アルゴリズムの性能に影響を及ぼす可能性がある．

我々は，$r_{\text{cost}}$の値を決める代わりに，エージェントが終了状態に到達する頻度を制御する手法を提案する．
終了状態に到達する可能性があるMDPに対して，環境のResetのみを導入し，Reset Costを加えない新たなMDPを考える．(つまり$r_{\text{cost}}=0$としたときの環境と同義である．)
元のMDPにおける終了状態の集合を$\mathcal{S}_{\text{term}}$として，方策$\pi$でエピソードが終了状態に到達する頻度$\rho_{\text{reset}}^\pi$を以下のように定義する．
$$
  \begin{aligned}
    \rho_{\text{reset}}^\pi & = \lim_{T \rightarrow \infty} \frac{1}{T} \mathbb{E}_{\pi}{ \left[ \sum_{t=0}^\infty \mathbbm{1}\left(S_t \in \mathcal{S}_{\text{term}}\right) \right] } \\
                            & = \sum_{s \in \mathcal{S}} d_\pi(s) \mathbbm{1}\left(s \in \mathcal{S}_{\text{term}}\right)
  \end{aligned}
$$
である．
頻度$\rho_{\text{reset}}^\pi$を用いて，以下のような制約付き最適化問題を考える．
\begin{equation}
  \label{eq:reset_cost_optimization}
  \begin{aligned}
    %  & \max_{\pi}\sum_{s \in \mathcal{S}} d_\pi(s, a) r(s,a) \left(= \rho^\pi\right)                                                        \\
    %  & \text{s.t. }  \sum_{s \in \mathcal{S}} d_\pi(s) \mathbbm{1}\left(s \in \mathcal{S}_{\text{term}}\right) \leq \epsilon_{\text{reset}}
     & \max_{\pi} \rho^\pi                                               \\
     & \text{s.t. } \rho_{\text{reset}}^\pi \leq \epsilon_{\text{reset}}
  \end{aligned}
\end{equation}
この問題は，平均報酬を最大化するという目的関数に対して，エピソードが終了状態に到達する頻度を制御する制約条件を付けたものであり，$\epsilon_{\text{reset}} \in (0, 1)$はユーザーが設定するパラメーターである．

この制約付き最適化問題に強双対性を仮定し，Dual Gradient Descent(引用)を適用する．
Dual variableを$\lambda \geq 0$とし，Lagrangianを以下のように定義する．
$$
  \begin{aligned}
    \mathcal{L}(\pi, \lambda) & = \rho^\pi - \lambda \left( \rho_{\text{reset}}^\pi - \epsilon_{\text{reset}} \right)                                                                          \\
                              & = \sum_{s \in \mathcal{S}} d_\pi(s, a) \left(r(s,a) - \lambda \mathbbm{1}\left(s \in \mathcal{S}_{\text{term}}\right) - \lambda \epsilon_{\text{reset}}\right)
  \end{aligned}
$$
Dual Gradient Descentは，Lagrangianをprime variablesに関して最適化した後，dual variableの勾配更新を1ステップ行うという手法だが，
我々はSACの温度パラメータの自動調整\cite{Haarnoja2018SACv2}と同様，prime variablesに関する勾配更新とdual variableに関する勾配更新を1ステップ交互に行うこととする．

この問題でのprime variablesに関する更新は，$\rho^\pi - \lambda \rho_{\text{reset}}^\pi$の方策$\pi$に関する最大化の最適化ステップと等しい．
$\rho^\pi - \lambda \rho_{\text{reset}}^\pi$は，$r_{\text{cost}}=\lambda$として環境をResetした際の平均報酬と等しいため，
このステップは，\ref{sec:Average_Reward_Soft_Policy_Improvement_Theorem}節に従い方策$\pi$をReset付きの環境において更新することと等しい．

Dual variablesに関する更新は，$- \lambda \left(\rho_{\text{reset}}^\pi - \epsilon_{\text{reset}} \right)$の最小化の勾配ステップとなる．
すなわち，$\rho_{\text{reset}}^\pi > \epsilon_{\text{reset}}$の場合は，Reset Costにあたる$\lambda$は増大し，$\rho_{\text{reset}}^\pi < \epsilon_{\text{reset}}$の場合は減少する．
また，Resetが発生する頻度を表す$\rho_{\text{reset}}^\pi$の値は，報酬を$r(s,a) =  \mathbbm{1}\left(S_t \in \mathcal{S}_{\text{term}}\right)$と設定した場合の平均報酬と等しい．
そのため，$r(s,a) =  \mathbbm{1}\left(S_t \in \mathcal{S}_{\text{term}}\right)$とした場合のQ関数$Q_{\text{reset}}$を構成し，
\ref{sec:RVI_Q_learning_based_Q_Network_update}節で示した更新法により，$Q_{\text{reset}}$を更新することで，$\rho_{\text{reset}}^\pi$の値を推定することができる．
% 主問題を式\ref{eq:P}，双対問題を式\ref{eq:D}をのように書き表す．
% $$
%   \begin{aligned}
%     \max_{\pi} \min_{\lambda > 0} \underE{s \sim d_\mu \\a \sim \mu}{r(s,a) - \lambda( - \epsilon)}\label{eq:P}\\
%     %   \min_{\lambda > 0} \max_{\mu} \underE{s \sim d_\mu\\a \sim \mu}{r(s,a) - \lambda(\IsTerminal{s} - \epsilon)}\label{eq:D}
%   \end{aligned}
% $$


==> sections/ja/04_experiments.tex <==
\section{Experiment}

我々は，以下の実験で2つのことを確認する:
(1) RVI-SACと，割引率を用いたSAC\cite{Haarnoja2018SACv2}や既存のoff-policy average reward DRLであるARO-DDPG\cite{Saxena2023ARODDPG}の性能の比較．
(2) 我々の提案手法における，各構成要素がどのように性能に寄与しているか．
これを確認するために，Gymnasium\cite{towers_gymnasium_2023}で実装されたMuJoCo pysical simulator\cite{todorov2012mujoco}の6つのタスク(Ant, HalfCheetah, Hopper, Walker2d, Humanoid, Swimmer)を用いてベンチマーク実験を行った．
ここで，SwimmerとHalfCheetah環境には，終了状態が設定されていないため，Resetが発生しないことに注意する．

\subsection{Comparative evaluation}
\label{sec:comparative_evaluation}

\begin{figure*}[t]
    \begin{subfigure}{1.0\textwidth}
        \centering
        \includegraphics[scale=0.5]{plotter/figures/main_result/legend.png}
    \end{subfigure}
    \centering
    \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plotter/figures/main_result/Swimmer.png}
        \caption{Swimmer}
        \label{fig:main_result_swimmer}
    \end{subfigure}
    \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plotter/figures/main_result/Ant.png}
        \caption{Ant}
        \label{fig:main_result_ant}
    \end{subfigure}
    \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plotter/figures/main_result/Walker2d.png}
        \caption{Walker2d}
        \label{fig:main_result_walker2d}
    \end{subfigure}%

    \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plotter/figures/main_result/Humanoid.png}
        \caption{Humanoid}
        \label{fig:main_result_humanoid}
    \end{subfigure}
    \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plotter/figures/main_result/Hopper.png}
        \caption{Hopper}
        \label{fig:main_result_hopper}
    \end{subfigure}
    \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plotter/figures/main_result/HalfCheetah.png}
        \caption{HalfCheetah}
        \label{fig:main_result_halfcheetah}
    \end{subfigure}
    \caption{Learning curves for the Gymnasium continuous control tasks. The shaded region represents half a standard deviation of the
        average evaluation over 10 trials.}
    \label{fig:main_result}
\end{figure*}

% \begin{table*}[htp]
%     \centering
%     \caption{各試行の最大評価値の平均値と標準偏差}
%     \label{tab:main_result}
%     \scriptsize
%     \begin{tabular}{lllllll}
%         \toprule
%                     & RVI-SAC          & SAC($\gamma = 0.99$) & SAC($\gamma = 0.999$) & SAC($\gamma = 0.97$) & ARO-DDPG       & ATRPO          \\
%         \midrule
%         Swimmer     & 344.04±3.07      & 75.99±31.38          & 313.31±89.89          & 51.12±0.75           & 249.23±135.60  & 363.67±0.60    \\
%         Walker2d    & 5002.94±621.59   & 4645.56±454.69       & 2304.99±868.53        & 2588.68±1293.16      & 2351.35±683.16 & 1768.99±429.67 \\
%         Humanoid    & 8335.98±278.81   & 5483.13±85.23        & 5218.07±95.59         & 6390.71±1118.50      & 5185.16±115.91 & 471.37±46.04   \\
%         Ant         & 6102.90±289.68   & 4511.20±605.98       & 1948.53±875.50        & 4855.87±1257.02      & 2178.45±271.49 & 959.3±18.57    \\
%         Hopper      & 3413.17±165.09   & 3427.3±140.58        & 2325.69±280.54        & 787.12±62.76         & 1509.60±444.62 & 3242.44±131.16 \\
%         HalfCheetah & 11011.71±1419.09 & 11429.99±229.85      & 9939.07±625.93        & 11165.22±1054.20     & 7206.28±715.92 & 1134.57±205.30 \\
%         \bottomrule
%     \end{tabular}
% \end{table*}

我々は，それぞれのアルゴリズムに対して，乱数シードの異なる10試行の実験を行い，5000ステップおきに評価値をサンプルした．
SAC/RVI-SACでは，評価時には確率的方策を決定的方策として扱う．
トレーニング時と評価時の打ち切りステップ数を両方1000に設定する．
図\ref{fig:main_result}は，RVI-SACと，様々な割引率をもつSAC，ARO-DDPGの学習曲線を示しす．
この実験では，評価値を1000ステップの報酬の合計値(total\_reward)に設定している．
評価値をaverage reward(total\_reward / survival\_step)に設定した場合の実験結果はAppendix. \ref{sec:appendix_main_result}に示す．
% 指標について詳しく説明する．

RVI-SACと様々な割引率を設定したSACを比較すると，RVI-SACがHalfCheetahを除く全ての環境で最も良い割引率を持つSACやARO-DDPG以上の性能を示している．
注目すべきはSwimmer環境における実験結果(図\ref{fig:main_result_swimmer})である．
Swimmer環境以外では，SACの割引率の推奨値とされる\cite{Haarnoja2018SAC}$\gamma = 0.99$が他の割引率よりもよい性能を示しているが，Swimmer環境では，$\gamma = 0.999$という推奨値よりも高い割引率を設定することが必要である．
しかし，高い割引率を設定することは，学習の不安定化や遅い収束を引き起こす可能性が指摘されており\cite{Fujimoto2018TD3,Dewanto2021ExaminingAR}，実際にSwimmer以外の環境では$\gamma = 0.999$という設定は低い性能を示す．
それと比べて，RVI-SACは，Swimmer環境では$\gamma = 0.999$以上の性能を示し，他の環境では$\gamma = 0.99$以上の性能を示している．
この結果は，従来の割引率を用いたSACでは，割引率の設定と，それによる報酬和の歪みが，性能に大きく影響する可能性があるのに対して，
RVI-SACでは，平均報酬を用いるため，そのような問題が発生しないことを示している．

% 全体的にという表現をもっと具体的にする．
RVI-SACとARO-DDPGを比較すると，全ての環境でRVI-SACが高い性能を示している．
これはRVI-SACは割引率を用いたSACと同様に，報酬にエントロピー項を含めることによる効果によって，決定的方策を用いるARO-DDPGと比べて高い性能を示していると考えられる．

\subsection{Design evaluation}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plotter/figures/sac_with_reset/Ant-ablation.png}
        % \caption{Discounted SAC with Reset. 赤はRVI-SACを，青はDiscounted SACに環境のResetを導入したものを示している．}
        \caption{Perfomance Comparison with SAC with Reset}
        \label{fig:sac_with_reset}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plotter/figures/rvi_ablation/rvi_ablation.png}
        \caption{Ablation Study of Delayed f(Q) Update}
        \label{fig:rvi_ablation}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plotter/figures/fixed_reset/fixed_reset.png}
        \caption{Fixed Reset Cost}
        \label{fig:fixed_reset}
    \end{subfigure}
    \caption{
        Experimental results demonstrating the effectiveness of each component of RVI-SAC.
        The three graphs all represent learning curves for the Ant environment. They compare RVI-SAC (red) with:
        \textbf{(a)} SAC (blue) incorporating environment reset and automatic adjustment of Reset Cost,
        \textbf{(b)} Variants using Reference States $(s,a)-\#1$ (blue) and $(s,a)-\#2$ (green) instead of Delayed f(Q) Update, and a direct application of Equation \ref{eq:F_Sampled} (yellow),
        \textbf{(c)} Versions with fixed Reset Costs set to 100 (blue), 250 (green), and 10 (yellow).
    }
\end{figure*}
% captionを詳しく書く．


前節で我々は，RVI-SACが，割引率を用いた従来のSACと比べて全体的に良い性能を示すことを示した．
本節で我々は，RVI-SACの各構成要素が全体の性能にどのように寄与しているかを示す．

% TODO:タイトルを全体的に何をやりたいのかが明確にわかりやすい

% TODO:Reset抜きでも平均報酬型強化学習に有効性があることを明確に書く
\textbf{Perfomance Comparison with SAC and ARO-DDPG with Reset}

RVI-SACは，環境のResetと自動調整されたReset Costを導入しているため，termination後の報酬を0と設定しているSAC/ARO-DDPGとは，異なる報酬の構造を用いている．
そこで，RVI-SACとReset Costの自動調整を導入したSAC/ARO-DDPGの性能比較実験を行うことで，同じ報酬構造を用いたときのRVI-SACの性能を確認する．
図\ref{fig:sac_with_reset}は，RVI-SACとReset Costの自動調整を導入したSACのAnt環境における学習曲線を示している．
(他環境に対する実験結果はAppendix. \ref{sec:appendix_sac_with_reset}に示す．)
ここで，SACにおいては，割引率として\cite{Haarnoja2018SAC}で推奨されている$\gamma = 0.99$を用いている．

この結果より，RVI-SACのほうが，Reset Costを導入したSACよりも高い性能を示していることがわかる．
よって，RVI-SACが従来のSACと比べて高い性能を示すのは，Reset Costの導入による報酬の構造の違いによるものではなく，平均報酬を用いたことによる効果であることが推測される．

\textbf{Ablation Study of Delayed f(Q) Update}

\ref{sec:RVI_Q_learning_based_Q_Network_update}節で提案したDelayd f(Q) Updateの有効性を検証する実験を行う．
この手法は，Q関数の更新を特定の状態行動ペアに依存させることなく，安定して学習を行うためのものであり，この工夫の有効性を検証するためには2つのことを確認する:
(1) 関数$f(Q)$の選択として，特定の状態行動ペア$(S,A)$に依存する$f(Q) = Q(S,A)$を選択した場合，この選択によって性能が依存する場合があること．
(2) 式\ref{eq:F_Sampled}を用いてQ関数を更新した場合，学習が不安定になること．
これを，確認するために，3パターンのアルゴリズムの性能比較を行った:
(1) RVI-SAC
(2) Reference Stateとして，ランダムに行動した際に得られる状態行動ペアを二種類($(s,a)-\#1, (s,a)-\#2$)サンプルし，$f(Q) = Q(s,a)$としてQ関数を更新する手法
(3) 式\ref{eq:F_Sampled}を用いてQ関数を更新する手法


%TODO: RVI-SAC Without Resetという文言をどこかに出しておく
%TODO: 式６とは何かの簡単な説明を入れる
図\ref{fig:rvi_ablation}は，これらの手法のAnt環境における学習曲線を示している．
まず，Reference Stateを用いた手法とRVI-SACとの比較に関して，$(s,a)-\#1$を用いる場合は，RVI-SACと同等の性能を示しているが，$(s,a)-\#2$を用いる場合は，RVI-SACよりも学習が遅いことがわかる．
この実験結果より，Reference Stateを用いた手法においては，Reference Stateの選択によって性能が依存することがわかる．
次に，式\ref{eq:F_Sampled}を用いた手法とRVI-SACとの比較に関して，式\ref{eq:F_Sampled}を用いた手法は，RVI-SACよりも非常に低い性能を示している．
これより，RVI-SACではDelayd f(Q) Updateを用いることで，学習が安定し，高い性能を示してるということが推測される．
以上より，特定の状態行動ペアに依存せず，安定したQ関数の更新を行うDelayd f(Q) Updateの有効性が示唆された．%(suggest)


\textbf{Fixed Reset Cost}

\ref{sec:Automatic_Reset_Cost_Adjustment}節で提案したReset Costの自動調整の有効性を検証する実験を行う．
ATRPO\cite{Yiming2021ATRPO}においては，Reset Costが固定されており推奨値が100と設定されていた．
しかし，適切なReset Costの値は，タスクや手法によって異なることが懸念されるため，Reset Costの自動調整を提案した．
我々は，この機構の有効性を示すために，Ant環境において，Reset Costを固定した場合と，自動調整した場合の学習曲線を比較した．

図\ref{fig:fixed_reset}は，これらの手法のAnt環境における学習曲線を示している．
$r_{\text{cost}} = N$という凡例があるものが，Reset Costを$N$に固定した場合の学習曲線である．
この結果より，ATRPOの推奨値である$r_{\text{cost}} = 100$とすると，RVI-SACよりも性能が低くなり，$r_{\text{cost}} = 10$と設定した場合がRVI-SACとほぼ同等，$r_{\text{cost}} = 250$と設定すると大きく性能が低下することがわかる．
以上の実験結果より，Reset Costの値によって性能が大きく変わる可能性があることが示され，Reset Costの自動調整によって，良いReset Costを設定した場合と同等の性能を示すことがわかる．

==> sections/ja/05_related_works.tex <==
\section{Related Works}

continuing taskに平均報酬基準を用いることの有効性が指摘されている．
\citet{Blackwell1962DiscreteDP}は，平均報酬を最大化するBlackwell optimal policy $\pi^*$が存在し，$\gamma \geq \gamma^*$を満たす割引報酬基準に対して最適な方策はBlackwell optimal policyと一致することを示した．
しかし，\cite{Dewanto2021ExaminingAR}は，$\gamma \geq \gamma^*$を満たすように大きい割引率を設定することは，収束速度を遅くすること，割引率を小さく設定することはsuboptimalなpolicyにつながる可能性があることを示し，
更にrecurrent MDPsに平均報酬基準を直接用いることは，初期状態に依存しない最適方策を得ることができる，高い収束率, 学習目的とperfomance metricsの不一致の少なさという点でメリットがあることが示されている．
また，\cite{Naik2019DRLOptimization}では，関数近似を伴う割引強化学習は最適化問題ではなく，最適方策が定義されないという問題を指摘している．

平均報酬基準のtabular Q-learning手法や理論的な分析\cite{Schwartz1993RLearning,Singh1999RLearning,Abounadi2001RVI,Wan2020DifferentialQLearning,Yang2016CSVQLearning}は，割引報酬基準のそれらと比べて少ないものの，いくつかの研究がある．
我々の提案手法のベースとなった手法の一つであるRVI Q-learningは\citet{Abounadi2001RVI}によって提案され\cite{Wan2020DifferentialQLearning}によって関数$f$に関して一般化された．
RVI Q-learningに関連するアルゴリズムとして，RVI Q-learningのspecial caseであるDiffrential Q-learning\cite{Wan2020DifferentialQLearning}がある．
これらの手法は\citet{Wan2022OConvergenceWeaklyMDPs}によってweakly communicating MDPsにおいてもasymptotic convergenceが示されている．

平均報酬基準において，function-approximationにfocusした手法もいくつか提案されてきた．
特に\citet{Saxena2023ARODDPG}はDDPGを平均報酬基準に拡張した研究であり，我々の提案手法との関わりが深く，dm-controlを用いた実験において，その有効性を示した．
更に，この研究は，Linear Function Approximationにおいてのasymptotic convergenceとfinite time analysisを提供しており，将来的に我々の提案手法にもこのような分析が期待される．
他には，POLITEX\cite{Chaudhuri2019POLITEX}ではPOLITEXは，以前のポリシーの行動価値関数推定値の合計に対するボルツマン分布を用いてポリシーを更新する手法であり，Atariを用いた実験で性能を示した．
また，ATRPO\cite{Yiming2021ATRPO}/APO\cite{Xiaoteng2021APO}は，on-policy settingにおけるpolicy improvement boundに基づきポリシーを更新する手法であり，Mujocoを用いた実験で高い性能を示した．

